Interpretable and intervenable ultrasonography-based machine learning models for pediatric appendicitis

Appendicitis is among the most frequent reasons for pediatric abdominal surgeries. Previous decision support systems for appendicitis have focused on clinical, laboratory, scoring, and computed tomography data and have ignored abdominal ultrasound, despite its noninvasive nature and widespread availability. In this work, we present interpretable machine learning models for predicting the diagnosis, management and severity of suspected appendicitis using ultrasound images. Our approach utilizes concept bottleneck models (CBM) that facilitate interpretation and interaction with high-level concepts understandable to clinicians. Furthermore, we extend CBMs to prediction problems with multiple views and incomplete concept sets. Our models were trained on a dataset comprising 579 pediatric patients with 1709 ultrasound images accompanied by clinical and laboratory data. Results show that our proposed method enables clinicians to utilize a human-understandable and intervenable predictive model without compromising performance or requiring time-consuming image annotation when deployed. For predicting the diagnosis, the extended multiview CBM attained an AUROC of 0.80 and an AUPR of 0.92, performing comparably to similar black-box neural networks trained and tested on the same dataset.

==> src/chapters/extended_data.tex <==
\section*{Extended data}

\setcounter{figure}{0}
\renewcommand{\thefigure}{\arabic{figure}}
\renewcommand{\figurename}{Extended Data Fig.}

\setcounter{table}{0}
\renewcommand{\thetable}{\arabic{table}}
\renewcommand{\tablename}{Extended Data Table}

\input{src/tables/predictive_perf_mvawa.tex}

\input{src/tables/concept_disambiguation.tex}

\begin{figure}[h!]%
\centering
\includegraphics[width=0.9\textwidth]{src/figures/preproc_example.pdf}
\caption{An example of multiple US images acquired from a single patient from the pediatric appendicitis dataset. For this patient, views I and \mbox{II} correspond to longitudinal and transverse sections of the appendix, respectively; view \mbox{III} depicts the reaction in tissue surrounding the appendix. Original images \mbox{(\emph{left})} contain graphical interface elements and expert-made markers, whereas preprocessed images \mbox{(\emph{right})} have been inpainted, cropped, and padded.  }\label{fig:us_example}
\end{figure}

\input{src/tables/concepts_management.tex}

\input{src/tables/concepts_severity.tex}

\begin{landscape}
\begin{figure}[h!]%
\centering
\includegraphics[width=1.4\textwidth]{src/figures/online_tool_schematic.pdf}
\caption{An illustrated use case for the pediatric appendicitis online prediction tool. \mbox{(1) The} user uploads input ultrasound images corresponding to a single patient. \mbox{(2) Optionally,} preprocessing is performed, and the tool displays original and preprocessed US images. \mbox{(3) The} tool displays predicted concept values alongside predicted value histograms obtained from the training data. The user can compare current predictions to those made for labeled training data points. \mbox{(4) The} tool shows the prediction for the target variable, i.e. for the diagnosis. \mbox{(5) The} user may choose to intervene on the concept predictions and, thus, affect the target prediction. In this example, concept predictions that were intervened on are indicated by yellow dotted lines.}\label{fig:tool_gui}
\end{figure}
\end{landscape}

\clearpage

\newpage

==> src/tables/ablation_results.tex <==
\begin{minipage}{\textwidth}
    \footnotesize
    \begin{center}
        \begin{tabular}{llm{1.8cm}cm{1.8cm}c}
            \toprule
            \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{AUROC}} & \multirow{2}{*}{$\mathrm{median}\: \left\vert\widehat{\mathrm{corr}}\left(\hat{c}_i,\hat{z}_j\,\vert\,y=k\right)\right\vert$} \\
            \cmidrule{3-5} &
            & \multicolumn{1}{c}{\textbf{Target}} & & \multicolumn{1}{c}{\textbf{Concepts}} \\
            \toprule
            \multirow{4}{*}{Synthetic} & MVCBM & \tentry{0.605}{0.029} &  & \tentry{0.756}{0.020} & --- \\
            & SSMVCBM, $\lambda=0$ & \tentry{0.640}{0.020} &  & \tentry{0.756}{0.020} &  0.059; [0.045, 0.075] \\
            & SSMVCBM, $\lambda=0.01$ & \tentry{0.638}{0.020} &  & \tentry{0.756}{0.020} & 0.059; [0.043, 0.082] \\
            & SSMVCBM, $\lambda=0.1$ & \tentry{0.629}{0.014} &  & \tentry{0.756}{0.020} & 0.052; [0.040, 0.063] \\
            \midrule
            \multirow{4}{*}{MVAwA} & MVCBM & \tentry{0.893}{0.009} &  &\tentry{0.957}{0.006} & --- \\
            & SSMVCBM, $\lambda=0$ & \tentry{0.963}{0.011} &  & \tentry{0.957}{0.006} & 0.114; [0.109, 0.120]\\
            & SSMVCBM, $\lambda=0.01$ & \tentry{0.946}{0.008} &  & \tentry{0.957}{0.006} & 0.105; [0.097, 0.116] \\
            & SSMVCBM, $\lambda=0.1$ & \tentry{0.927}{0.011} &  & \tentry{0.957}{0.006} & 0.071; [0.056, 0.081] \\
            \bottomrule
        \end{tabular}
    \end{center}
    \vspace{0.5cm}
\end{minipage}

==> src/tables/architectures.tex <==
\begin{table}[h!]
    \footnotesize
    \centering
    \caption{Summary of the MVCBM architectures used for the \mbox{(a) synthetic} and \mbox{(b) MVAwA} and pediatric appendicitis datasets. Here, $B$ denotes the batch size, $V$ is the maximum number of views, $w$ and $h$ are the width and height of the input image, $K$ is the number of concepts, $H$ is the number of units in the hidden layer of $f_{\boldsymbol{\theta}}(\cdot)$, and $N_o$ is the number of output units. \label{tab:architectures}}

    \subfigure[]{
        \centering
        \begin{tabular}{clll}
            \textbf{Module} & \textbf{Layers} & \textbf{Input Dimensions} & \textbf{Output Dimensions}\\
            \toprule
            \multirow{10}{.5cm}{$\boldsymbol{h}_{\boldsymbol{\psi}}(\cdot)$} & \texttt{Linear} & ($B$, $V$, 500) & ($B$, $V$, 256) \\
            & \texttt{Dropout(0.05)} & ($B$, $V$, 256) & ($B$, $V$, 256) \\
            & \texttt{BatchNorm1d} & ($B$, $V$, 256) & ($B$, $V$, 256) \\
            & \texttt{Linear} & ($B$, $V$, 256) & ($B$, $V$, 256) \\
            & \texttt{Dropout(0.05)} & ($B$, $V$, 256) & ($B$, $V$, 256) \\
            & \texttt{BatchNorm1d} & ($B$, $V$, 256) & ($B$, $V$, 256) \\
            & \texttt{Linear} & ($B$, $V$, 256) & ($B$, $V$, 256) \\
            & \texttt{Dropout(0.05)} & ($B$, $V$, 256) & ($B$, $V$, 256) \\
            & \texttt{BatchNorm1d} & ($B$, $V$, 256) & ($B$, $V$, 256) \\
            & \texttt{Linear} & ($B$, $V$, 256) & ($B$, $V$, 128) \\
            \midrule
            $\boldsymbol{r}_{\boldsymbol{\xi}}(\cdot)$ & \texttt{LSTM}/\texttt{mean} & ($B$, $V$, 128) & ($B$, 128)\\
            \midrule
            \multirow{6}{.5cm}{$\boldsymbol{s}_{\boldsymbol{\zeta}}(\cdot)$} & \texttt{Linear} & ($B$, 128) & ($B$, 256)\\
            & \texttt{ReLu} & ($B$, 256) & ($B$, 256)\\
            & \texttt{Linear} & ($B$, 256) & ($B$, 64)\\
            & \texttt{ReLu} & ($B$, 64) & ($B$, 64)\\
            & \texttt{Linear} & ($B$, 64) & ($B$, $K$)\\
            & \texttt{Sigmoid} & ($B$, $K$) & ($B$, $K$)\\
            \midrule
            \multirow{4}{.5cm}{$f_{\boldsymbol{\theta}}(\cdot)$}
            & \texttt{Linear} & ($B$, $K$) & ($B$, $H$)\\
            & \texttt{ReLu} & ($B$, $H$) & ($B$, $H$)\\
            & \texttt{Linear} & ($B$, $H$) & ($B$, 1)\\
            & \texttt{Sigmoid} & ($B$, 1) & ($B$, 1)\\
            \bottomrule
        \end{tabular}
    }

    \vspace{1.0cm}
    
    \subfigure[]{
        \centering
        \begin{tabular}{clll}
            \textbf{Module} & \textbf{Layers} & \textbf{Input Dimensions} & \textbf{Output Dimensions}\\
            \toprule
            $\boldsymbol{h}_{\boldsymbol{\psi}}(\cdot)$ & \texttt{ResNet-18} & ($B$, $V$, 3, $w$, $h$) & ($B$, $V$, 512) \\
            \midrule
            $\boldsymbol{r}_{\boldsymbol{\xi}}(\cdot)$ & \texttt{LSTM}/\texttt{mean} & ($B$, $V$, 512) & ($B$, 512)\\
            \midrule
            \multirow{6}{.5cm}{$\boldsymbol{s}_{\boldsymbol{\zeta}}(\cdot)$} & \texttt{Linear} & ($B$, 512) & ($B$, 256)\\
            & \texttt{ReLu} & ($B$, 256) & ($B$, 256)\\
            & \texttt{Linear} & ($B$, 256) & ($B$, 64)\\
            & \texttt{ReLu} & ($B$, 64) & ($B$, 64)\\
            & \texttt{Linear} & ($B$, 64) & ($B$, $K$)\\
            & \texttt{Sigmoid} & ($B$, $K$) & ($B$, $K$)\\
            \midrule
            \multirow{4}{.5cm}{$f_{\boldsymbol{\theta}}(\cdot)$}
            & \texttt{Linear} & ($B$, $K$) & ($B$, $H$)\\
            & \texttt{ReLu} & ($B$, $H$) & ($B$, $H$)\\
            & \texttt{Linear} & ($B$, $H$) & ($B$, $N_o$)\\
            & \texttt{Sigmoid}/\texttt{Softmax} & ($B$, $N_o$) & ($B$, $N_o$)\\
            \bottomrule
        \end{tabular}
    }
\end{table}

==> src/tables/concept_disambiguation.tex <==
\begin{table}[h!]
\centering
\caption{Explanation and descriptive statistics for the concept variables chosen for the pediatric appendicitis dataset. The right-most column reports the percentage of the positive outcome values.}
\label{tab:concept_distribution}
    \begin{tabular}{cp{4.5cm}p{8cm}r} 
        \toprule
        & \textbf{Name} & \textbf{Description} & \textbf{Pos., \%} \\[0.5ex] 
        \toprule
        $c_1$ & Visibility of the appendix & visibility of the vermiform appendix during the examination & 76 \\
        \midrule
        $c_2$ & Free intraperitoneal fluid & free fluids in the abdomen & 43 \\
        \midrule
        $c_3$ & Appendix layer structure & characterization of the appendix layers, e.g. irregular in case of an increasing inflammation & 14 \\
        \midrule
        $c_4$ & Target sign & axial image of the appendix with the fluid-filled center surrounded by echogenic mucosa and submucosa and hypoechoic muscularis & 13 \\
        \midrule
        $c_5$ & Surrounding tissue reaction & inflammation signs in tissue surrounding the appendix  & 33 \\ 
        \midrule
        $c_6$ & Pathological lymph nodes & enlarged and inflamed intra-abdominal lymph nodes   & 21 \\
        \midrule
        $c_7$ & Thickening of the bowel wall & edema of the intestinal wall, $>$ 2--3 mm & 8 \\
        \midrule
        $c_8$ & Coprostasis & fecal impaction in the colon & 6 \\
        \midrule
        $c_9$ & Meteorism & accumulation of gas in the intestine & 15 \\
        
        
        \bottomrule
    \end{tabular}
\end{table}

==> src/tables/concepts_diagnosis.tex <==
\begin{landscape}
\begin{table*}[h]
    \footnotesize
    \begin{center}
    \caption{Models' test-set performance at concept prediction on the pediatric appendicitis dataset with the diagnosis as the target variable. Test-set AUROCs and AUPRs are reported as averages and standard deviations across ten independent initializations. Herein, ``seq'' and ``joint'' denote sequential and joint optimization, respectively, whereas ``avg'' and ``LSTM'' stand for the averaging- and LSTM-based fusion. AUROCs and AUPRs that are significantly greater than the expected performance of a fair coin flip (random) are marked by ``\textsuperscript{\textbf{*}}''. Bold indicates the best result; italics indicates the second best. The meaning of the concept variables: $c_1$, visibility of the appendix; $c_2$, free intraperitoneal fluid; $c_3$, appendix layer structure; $c_4$, target sign; $c_5$, surrounding tissue reaction; $c_6$, pathological lymph nodes; $c_7$, thickening of the bowel wall; $c_8$, coprostasis; $c_9$, meteorism.}
    \label{tab:appendicitis_concept_res} 
    \begin{tabular}{p{1.0cm}lp{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}}
        \toprule
        \multirow{2}{*}{\raisebox{-\heavyrulewidth}{\textbf{Metric}}} & \multirow{2}{*}{\raisebox{-\heavyrulewidth}{\textbf{Model}}} & \multicolumn{9}{c}{\textbf{Concept}}\\
        \cmidrule{3-11} & & $c_1$ & $c_2$ & $c_3$ & $c_4$ & $c_5$ & $c_6$ & $c_7$ & $c_8$ & $c_9$ \\
        \toprule
        \multirow{11}{20mm}{\textbf{AUROC}}
        & \multicolumn{1}{l}{Random} & 0.50 & 0.50 & 0.50 & 0.50 & 0.50 & 0.50 & 0.50 & 0.50 & 0.50 \\
        \cmidrule{2-11} & \multicolumn{1}{l}{CBM-seq} & \tentry{0.52}{0.04} & \tentry{0.47}{0.04} & \tentry{0.60}{0.07}\textsuperscript{\textbf{*}} & \tentry{0.56}{0.08} & \tentry{0.63}{0.05}\textsuperscript{\textbf{*}} & \tentry{0.57}{0.05}\textsuperscript{\textbf{*}} & \tentry{0.45}{0.08} & \tentry{0.48}{0.08} & \tentry{0.39}{0.07} \\
        & \multicolumn{1}{l}{CBM-joint} & \tentry{0.50}{0.05} & \tentry{0.47}{0.03} & \tentry{0.57}{0.05}\textsuperscript{\textbf{*}} & \tentry{0.54}{0.06} & \tentry{0.64}{0.04}\textsuperscript{\textbf{*}} & \tentry{0.59}{0.05}\textsuperscript{\textbf{*}} & \tentry{0.39}{0.06} & \tentry{0.57}{0.12} & \tentry{0.38}{0.09} \\
        \cmidrule{2-11} & \multicolumn{1}{l}{MVCBM-seq-avg} & \tentry{0.61}{0.05}\textsuperscript{\textbf{*}} & \tentry{0.49}{0.05} & \tentry{0.66}{0.08}\textsuperscript{\textbf{*}} & \tentry{0.60}{0.08}\textsuperscript{\textbf{*}} & \tentry{0.51}{0.08} & \tentry{0.66}{0.08}\textsuperscript{\textbf{*}} & \textit{\tentry{0.50}{0.04}} & \tentry{0.47}{0.12} & \tentry{0.55}{0.07} \\
        & \multicolumn{1}{l}{MVCBM-seq-LSTM}   & \textit{\tentry{0.83}{0.03}\textsuperscript{\textbf{*}}} & \textit{\tentry{0.59}{0.03}\textsuperscript{\textbf{*}}} & \tentry{0.62}{0.04}\textsuperscript{\textbf{*}} & \textbf{\tentry{0.71}{0.04}\textsuperscript{\textbf{*}}} & \tentry{0.65}{0.04}\textsuperscript{\textbf{*}} & \tentry{0.67}{0.07}\textsuperscript{\textbf{*}} & \tentry{0.49}{0.07} & \textbf{\tentry{0.68}{0.10}\textsuperscript{\textbf{*}}} & \textit{\tentry{0.73}{0.06}\textsuperscript{\textbf{*}}} \\
        & \multicolumn{1}{l}{MVCBM-joint-avg}   & \tentry{0.55}{0.10} & \tentry{0.47}{0.07} & \textbf{\tentry{0.73}{0.07}\textsuperscript{\textbf{*}}} & \tentry{0.63}{0.07}\textsuperscript{\textbf{*}} & \tentry{0.61}{0.06}\textsuperscript{\textbf{*}} & \tentry{0.63}{0.07}\textsuperscript{\textbf{*}} & \tentry{0.48}{0.06} & \tentry{0.45}{0.13} & \tentry{0.54}{0.11} \\
        & \multicolumn{1}{l}{MVCBM-joint-LSTM} & \textbf{\tentry{0.85}{0.03}\textsuperscript{\textbf{*}}} & \tentry{0.55}{0.04}\textsuperscript{\textbf{*}} & \tentry{0.58}{0.04}\textsuperscript{\textbf{*}} & \textit{\tentry{0.70}{0.03}\textsuperscript{\textbf{*}}} & \textbf{\tentry{0.75}{0.02}\textsuperscript{\textbf{*}}} & \tentry{0.55}{0.09} & \tentry{0.45}{0.12} & \tentry{0.68}{0.17} & \textbf{\tentry{0.77}{0.03}\textsuperscript{\textbf{*}}} \\
        \cmidrule{2-11} & \multicolumn{1}{l}{SSMVCBM-avg} & \tentry{0.62}{0.05}\textsuperscript{\textbf{*}} & \textbf{\tentry{0.60}{0.05}\textsuperscript{\textbf{*}}} & \textit{\tentry{0.72}{0.05}\textsuperscript{\textbf{*}}} & \tentry{0.67}{0.05}\textsuperscript{\textbf{*}} & \tentry{0.54}{0.05} & \textit{\tentry{0.68}{0.08}\textsuperscript{\textbf{*}}} & \textbf{\tentry{0.53}{0.11}} & \tentry{0.43}{0.08} & \tentry{0.47}{0.07} \\
        & \multicolumn{1}{l}{SSMVCBM-LSTM} & \textbf{\tentry{0.85}{0.04}\textsuperscript{\textbf{*}}} & \tentry{0.58}{0.06}\textsuperscript{\textbf{*}} & \tentry{0.66}{0.05}\textsuperscript{\textbf{*}} & \textbf{\tentry{0.71}{0.06}\textsuperscript{\textbf{*}}} & \textit{\tentry{0.67}{0.04}\textsuperscript{\textbf{*}}} & \textbf{\tentry{0.69}{0.06}\textsuperscript{\textbf{*}}} & \tentry{0.45}{0.09} & \textit{\tentry{0.66}{0.11}\textsuperscript{\textbf{*}}} & \textit{\tentry{0.73}{0.05}\textsuperscript{\textbf{*}}} \\
        \midrule
        \multirow{11}{20mm}{\textbf{AUPR}}
        & \multicolumn{1}{l}{Random} & 0.72 & 0.49 & 0.19 & 0.23 & 0.51 & 0.26 & 0.16 & 0.13 & 0.14 \\
        \cmidrule{2-11} & \multicolumn{1}{l}{CBM-seq} & \tentry{0.71}{0.03} & \tentry{0.53}{0.03}\textsuperscript{\textbf{*}} & \tentry{0.29}{0.06}\textsuperscript{\textbf{*}} & \tentry{0.26}{0.05} & \tentry{0.64}{0.05}\textsuperscript{\textbf{*}} & \tentry{0.38}{0.06}\textsuperscript{\textbf{*}} & \tentry{0.15}{0.03} & \tentry{0.12}{0.02} & \tentry{0.11}{0.02} \\
        & \multicolumn{1}{l}{CBM-joint} & \tentry{0.73}{0.05} & \tentry{0.49}{0.04} & \tentry{0.30}{0.06}\textsuperscript{\textbf{*}} & \tentry{0.30}{0.08} & \tentry{0.64}{0.05}\textsuperscript{\textbf{*}} & \tentry{0.38}{0.09}\textsuperscript{\textbf{*}} & \tentry{0.15}{0.05} & \tentry{0.19}{0.08} & \tentry{0.11}{0.02} \\
        \cmidrule{2-11} & \multicolumn{1}{l}{MVCBM-seq-avg} & \tentry{0.79}{0.04}\textsuperscript{\textbf{*}} & \tentry{0.53}{0.06} & \textit{\tentry{0.34}{0.10}\textsuperscript{\textbf{*}}} & \tentry{0.35}{0.10}\textsuperscript{\textbf{*}} & \tentry{0.53}{0.07} & \textit{\tentry{0.41}{0.07}\textsuperscript{\textbf{*}}} & \tentry{0.17}{0.04} & \tentry{0.14}{0.04} & \tentry{0.25}{0.12} \\
        & \multicolumn{1}{l}{MVCBM-seq-LSTM}   & \tentry{0.92}{0.02}\textsuperscript{\textbf{*}} & \textit{\tentry{0.59}{0.04}\textsuperscript{\textbf{*}}} & \tentry{0.32}{0.05} & \textbf{\tentry{0.38}{0.04}\textsuperscript{\textbf{*}}} & \textit{\tentry{0.67}{0.04}\textsuperscript{\textbf{*}}} & \textbf{\tentry{0.42}{0.10}\textsuperscript{\textbf{*}}} & \tentry{0.15}{0.02} & \textit{\tentry{0.21}{0.08}} & \textbf{\tentry{0.40}{0.11}\textsuperscript{\textbf{*}}} \\
        & \multicolumn{1}{l}{MVCBM-joint-avg} & \tentry{0.75}{0.08} & \tentry{0.48}{0.06} & \textbf{\tentry{0.38}{0.09}\textsuperscript{\textbf{*}}} & \tentry{0.30}{0.06} & \tentry{0.58}{0.05}\textsuperscript{\textbf{*}} & \tentry{0.39}{0.08}\textsuperscript{\textbf{*}} & \textbf{\tentry{0.21}{0.08}} & \tentry{0.15}{0.08} & \tentry{0.16}{0.05} \\
        & \multicolumn{1}{l}{MVCBM-joint-LSTM} & \textbf{\tentry{0.94}{0.01}\textsuperscript{\textbf{*}}} & \tentry{0.50}{0.05} & \tentry{0.26}{0.08} & \textit{\tentry{0.37}{0.07}\textsuperscript{\textbf{*}}} & \textbf{\tentry{0.74}{0.04}\textsuperscript{\textbf{*}}} & \tentry{0.32}{0.09} & \tentry{0.16}{0.08} & \textbf{\tentry{0.31}{0.20}} & \tentry{0.28}{0.07}\textsuperscript{\textbf{*}} \\
        \cmidrule{2-11} & \multicolumn{1}{l}{SSMVCBM-avg} & \tentry{0.79}{0.04}\textsuperscript{\textbf{*}} & \tentry{0.58}{0.03}\textsuperscript{\textbf{*}} & \textbf{\tentry{0.38}{0.05}\textsuperscript{\textbf{*}}} & \tentry{0.34}{0.04}\textsuperscript{\textbf{*}} & \tentry{0.54}{0.06} & \textbf{\tentry{0.42}{0.08}\textsuperscript{\textbf{*}}} & \textit{\tentry{0.20}{0.06}} & \tentry{0.12}{0.04} & \tentry{0.17}{0.07} \\
        & \multicolumn{1}{l}{SSMVCBM-LSTM} & \textit{\tentry{0.93}{0.03}\textsuperscript{\textbf{*}}} & \textbf{\tentry{0.60}{0.06}\textsuperscript{\textbf{*}}} & \tentry{0.31}{0.06}\textsuperscript{\textbf{*}} & \textbf{\tentry{0.38}{0.06}\textsuperscript{\textbf{*}}} & \textit{\tentry{0.67}{0.04}\textsuperscript{\textbf{*}}} & \tentry{0.39}{0.06}\textsuperscript{\textbf{*}} & \tentry{0.19}{0.06} & \tentry{0.19}{0.07} & \textit{\tentry{0.30}{0.09}\textsuperscript{\textbf{*}}} \\
        \bottomrule
    \end{tabular}
    \vspace{1cm}
    \end{center}
\end{table*}
\end{landscape}

==> src/tables/concepts_management.tex <==
\begin{landscape}
\begin{table*}[h!]
    \footnotesize
    \begin{center}
    \caption{Models' test-set performance at concept prediction on the appendicitis dataset with the management as the target variable. Test-set AUROCs and AUPRs are reported as averages and standard deviations across ten independent initializations. Herein, ``seq'' and ``joint'' denote sequential and joint optimization, respectively, whereas ``avg'' and ``LSTM'' stand for the averaging- and LSTM-based fusion. AUROCs and AUPRs that are significantly greater than the expected performance of a fair coin flip (random) are marked by ``\textsuperscript{\textbf{*}}''. Bold indicates the best result; italics indicates the second best. The meaning of the concept variables: $c_1$, visibility of the appendix; $c_2$, free intraperitoneal fluid; $c_3$, appendix layer structure; $c_4$, target sign; $c_5$, surrounding tissue reaction; $c_6$, pathological lymph nodes; $c_7$, thickening of the bowel wall; $c_8$, coprostasis; $c_9$, meteorism.}
    \label{tab:appendicitis_concept_res_management} 
    \begin{tabular}{p{1.0cm}lp{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}}
        \toprule
        \multirow{2}{*}{\raisebox{-\heavyrulewidth}{\textbf{Metric}}} & \multirow{2}{*}{\raisebox{-\heavyrulewidth}{\textbf{Model}}} & \multicolumn{9}{c}{\textbf{Concept}}\\
        \cmidrule{3-11} & & $c_1$ & $c_2$ & $c_3$ & $c_4$ & $c_5$ & $c_6$ & $c_7$ & $c_8$ & $c_9$ \\
        \toprule
        \multirow{11}{20mm}{\textbf{AUROC}}
        & \multicolumn{1}{l}{Random} & 0.50 & 0.50 & 0.50 & 0.50 & 0.50 & 0.50 & 0.50 & 0.50 & 0.50 \\
        \cmidrule{2-11} & \multicolumn{1}{l}{CBM-seq} & \tentry{0.51}{0.05} & \tentry{0.54}{0.07} & \tentry{0.63}{0.05}\textsuperscript{\textbf{*}} & \tentry{0.49}{0.07} & \tentry{0.65}{0.07}\textsuperscript{\textbf{*}} & \tentry{0.56}{0.06} & \tentry{0.47}{0.10} & \tentry{0.60}{0.10} & \tentry{0.54}{0.07} \\
        & \multicolumn{1}{l}{CBM-joint} & \tentry{0.54}{0.08} & \tentry{0.51}{0.08} & \tentry{0.64}{0.06}\textsuperscript{\textbf{*}} & \tentry{0.49}{0.06} & \textit{\tentry{0.67}{0.03}\textsuperscript{\textbf{*}}} & \tentry{0.54}{0.07} & \tentry{0.49}{0.07} & \tentry{0.56}{0.10} & \tentry{0.47}{0.09} \\
        \cmidrule{2-11} & \multicolumn{1}{l}{MVCBM-seq-avg} & \tentry{0.62}{0.06}\textsuperscript{\textbf{*}} & \tentry{0.48}{0.07} & \tentry{0.69}{0.03}\textsuperscript{\textbf{*}} & \tentry{0.54}{0.12} & \tentry{0.49}{0.08} & \tentry{0.60}{0.07}\textsuperscript{\textbf{*}} & \tentry{0.48}{0.09} & \tentry{0.47}{0.13} & \tentry{0.57}{0.09} \\
        & \multicolumn{1}{l}{MVCBM-seq-LSTM}   & \textbf{\tentry{0.86}{0.05}\textsuperscript{\textbf{*}}} & \textit{\tentry{0.55}{0.05}} & \tentry{0.62}{0.05}\textsuperscript{\textbf{*}} & \textit{\tentry{0.69}{0.03}\textsuperscript{\textbf{*}}} & \tentry{0.66}{0.04}\textsuperscript{\textbf{*}} & \textbf{\tentry{0.65}{0.06}\textsuperscript{\textbf{*}}} & \textit{\tentry{0.50}{0.07}} & \textbf{\tentry{0.75}{0.09}\textsuperscript{\textbf{*}}} & \textbf{\tentry{0.74}{0.06}\textsuperscript{\textbf{*}}} \\
        & \multicolumn{1}{l}{MVCBM-joint-avg}   & \tentry{0.52}{0.07} & \tentry{0.53}{0.06} & \textit{\tentry{0.71}{0.07}\textsuperscript{\textbf{*}}} & \tentry{0.59}{0.05}\textsuperscript{\textbf{*}} & \tentry{0.64}{0.07}\textsuperscript{\textbf{*}} & \textbf{\tentry{0.65}{0.04}\textsuperscript{\textbf{*}}} & \tentry{0.48}{0.10} & \tentry{0.54}{0.07} & \tentry{0.52}{0.15} \\
        & \multicolumn{1}{l}{MVCBM-joint-LSTM} & \tentry{0.80}{0.05}\textsuperscript{\textbf{*}} & \tentry{0.41}{0.08} & \tentry{0.66}{0.07}\textsuperscript{\textbf{*}} & \tentry{0.61}{0.04}\textsuperscript{\textbf{*}} & \tentry{0.66}{0.03}\textsuperscript{\textbf{*}} & \textit{\tentry{0.62}{0.07}\textsuperscript{\textbf{*}}} & \textbf{\tentry{0.51}{0.07}} & \tentry{0.62}{0.11} & \tentry{0.63}{0.08}\textsuperscript{\textbf{*}} \\
        \cmidrule{2-11} & \multicolumn{1}{l}{SSMVCBM-avg} & \tentry{0.62}{0.07}\textsuperscript{\textbf{*}} & \textbf{\tentry{0.57}{0.08}} & \textbf{\tentry{0.73}{0.04}\textsuperscript{\textbf{*}}} & \tentry{0.63}{0.05}\textsuperscript{\textbf{*}} & \tentry{0.55}{0.04} & \textbf{\tentry{0.65}{0.07}\textsuperscript{\textbf{*}}} & \textit{\tentry{0.50}{0.08}} & \tentry{0.49}{0.08} & \tentry{0.52}{0.05} \\
        & \multicolumn{1}{l}{SSMVCBM-LSTM} & \textit{\tentry{0.84}{0.02}\textsuperscript{\textbf{*}}} & \tentry{0.54}{0.05} & \tentry{0.70}{0.05}\textsuperscript{\textbf{*}} & \textbf{\tentry{0.70}{0.03}\textsuperscript{\textbf{*}}} & \textbf{\tentry{0.68}{0.05}\textsuperscript{\textbf{*}}} & \textit{\tentry{0.62}{0.07}\textsuperscript{\textbf{*}}} & \textit{\tentry{0.50}{0.10}} & \textit{\tentry{0.72}{0.05}\textsuperscript{\textbf{*}}} & \textit{\tentry{0.72}{0.10}\textsuperscript{\textbf{*}}} \\
        \midrule
        \multirow{11}{20mm}{\textbf{AUPR}}
        & \multicolumn{1}{l}{Random} & 0.72 & 0.49 & 0.19 & 0.23 & 0.51 & 0.26 & 0.16 & 0.13 & 0.14 \\
        \cmidrule{2-11} & \multicolumn{1}{l}{CBM-seq} & \tentry{0.76}{0.03} & \textit{\tentry{0.55}{0.07}} & \tentry{0.37}{0.09}\textsuperscript{\textbf{*}} & \tentry{0.23}{0.03} & \textit{\tentry{0.66}{0.07}\textsuperscript{\textbf{*}}} & \tentry{0.35}{0.10} & \textit{\tentry{0.19}{0.06}} & \tentry{0.20}{0.13} & \tentry{0.17}{0.03} \\
        & \multicolumn{1}{l}{CBM-joint} & \tentry{0.77}{0.04}\textsuperscript{\textbf{*}} & \tentry{0.51}{0.06} & \textbf{\tentry{0.45}{0.08}\textsuperscript{\textbf{*}}} & \tentry{0.24}{0.07} & \tentry{0.64}{0.04}\textsuperscript{\textbf{*}} & \tentry{0.29}{0.04} & \textit{\tentry{0.19}{0.05}} & \tentry{0.17}{0.09} & \tentry{0.15}{0.06} \\
        \cmidrule{2-11} & \multicolumn{1}{l}{MVCBM-seq-avg} & \tentry{0.79}{0.04}\textsuperscript{\textbf{*}} & \tentry{0.52}{0.08} & \tentry{0.35}{0.04}\textsuperscript{\textbf{*}} & \tentry{0.31}{0.14} & \tentry{0.51}{0.06} & \tentry{0.37}{0.08}\textsuperscript{\textbf{*}} & \tentry{0.17}{0.04} & \tentry{0.12}{0.04} & \tentry{0.18}{0.05} \\
        & \multicolumn{1}{l}{MVCBM-seq-LSTM}   & \textbf{\tentry{0.95}{0.02}\textsuperscript{\textbf{*}}} & \textit{\tentry{0.55}{0.03}\textsuperscript{\textbf{*}}} & \tentry{0.32}{0.08}\textsuperscript{\textbf{*}} & \textbf{\tentry{0.38}{0.04}\textsuperscript{\textbf{*}}} & \textit{\tentry{0.66}{0.03}\textsuperscript{\textbf{*}}} & \textit{\tentry{0.38}{0.09}\textsuperscript{\textbf{*}}} & \tentry{0.16}{0.02} & \textbf{\tentry{0.30}{0.16}} & \textbf{\tentry{0.30}{0.06}\textsuperscript{\textbf{*}}} \\
        & \multicolumn{1}{l}{MVCBM-joint-avg} & \tentry{0.71}{0.04} & \tentry{0.53}{0.05} & \tentry{0.36}{0.10}\textsuperscript{\textbf{*}} & \tentry{0.28}{0.03}\textsuperscript{\textbf{*}} & \tentry{0.60}{0.07}\textsuperscript{\textbf{*}} & \textbf{\tentry{0.39}{0.06}\textsuperscript{\textbf{*}}} & \tentry{0.17}{0.05} & \tentry{0.20}{0.07} & \tentry{0.21}{0.10} \\
        & \multicolumn{1}{l}{MVCBM-joint-LSTM} & \tentry{0.91}{0.03}\textsuperscript{\textbf{*}} & \tentry{0.44}{0.05} & \tentry{0.31}{0.06}\textsuperscript{\textbf{*}} & \tentry{0.33}{0.06}\textsuperscript{\textbf{*}} & \tentry{0.64}{0.03}\textsuperscript{\textbf{*}} & \textit{\tentry{0.38}{0.06}\textsuperscript{\textbf{*}}} & \textit{\tentry{0.19}{0.04}} & \tentry{0.19}{0.11} & \textit{\tentry{0.28}{0.14}} \\
        \cmidrule{2-11} & \multicolumn{1}{l}{SSMVCBM-avg} & \tentry{0.78}{0.06} & \textbf{\tentry{0.60}{0.07}\textsuperscript{\textbf{*}}} & \textit{\tentry{0.41}{0.08}\textsuperscript{\textbf{*}}} & \tentry{0.33}{0.08}\textsuperscript{\textbf{*}} & \tentry{0.55}{0.05} & \textbf{\tentry{0.39}{0.07}\textsuperscript{\textbf{*}}} & \textbf{\tentry{0.22}{0.06}} & \tentry{0.12}{0.02} & \tentry{0.23}{0.08} \\
        & \multicolumn{1}{l}{SSMVCBM-LSTM} & \textit{\tentry{0.93}{0.01}\textsuperscript{\textbf{*}}} & \textit{\tentry{0.55}{0.06}} & \tentry{0.38}{0.09}\textsuperscript{\textbf{*}} & \textit{\tentry{0.37}{0.06}\textsuperscript{\textbf{*}}} & \textbf{\tentry{0.67}{0.06}\textsuperscript{\textbf{*}}} & \tentry{0.35}{0.06}\textsuperscript{\textbf{*}} & \tentry{0.17}{0.05} & \textit{\tentry{0.24}{0.05}\textsuperscript{\textbf{*}}} & \tentry{0.27}{0.08}\textsuperscript{\textbf{*}} \\
        \bottomrule
    \end{tabular}
    \end{center}
\end{table*}
\end{landscape}

==> src/tables/concepts_severity.tex <==
\begin{landscape}
\begin{table*}[h!]
    \footnotesize
    \begin{center}
    \caption{Models' test-set performance at concept prediction on the appendicitis dataset with the severity as the target variable. Test-set AUROCs and AUPRs are reported as averages and standard deviations across ten independent initializations. Herein, ``seq'' and ``joint'' denote sequential and joint optimization, respectively, whereas ``avg'' and ``LSTM'' stand for the averaging- and LSTM-based fusion. AUROCs and AUPRs that are significantly greater than the expected performance of a fair coin flip (random) are marked by ``\textsuperscript{\textbf{*}}''. Bold indicates the best result; italics indicates the second best. The meaning of the concept variables: $c_1$, visibility of the appendix; $c_2$, free intraperitoneal fluid; $c_3$, appendix layer structure; $c_4$, target sign; $c_5$, surrounding tissue reaction; $c_6$, pathological lymph nodes; $c_7$, thickening of the bowel wall; $c_8$, coprostasis; $c_9$, meteorism.}
    \label{tab:appendicitis_concept_res_severity} 
    \begin{tabular}{p{1.0cm}lp{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}}
        \toprule
        \multirow{2}{*}{\raisebox{-\heavyrulewidth}{\textbf{Metric}}} & \multirow{2}{*}{\raisebox{-\heavyrulewidth}{\textbf{Model}}} & \multicolumn{9}{c}{\textbf{Concept}}\\
        \cmidrule{3-11} & & $c_1$ & $c_2$ & $c_3$ & $c_4$ & $c_5$ & $c_6$ & $c_7$ & $c_8$ & $c_9$ \\
        \toprule
        \multirow{11}{20mm}{\textbf{AUROC}}
        & \multicolumn{1}{l}{Random} & 0.50 & 0.50 & 0.50 & 0.50 & 0.50 & 0.50 & 0.50 & 0.50 & 0.50 \\
        \cmidrule{2-11} & \multicolumn{1}{l}{CBM-seq} & \tentry{0.51}{0.04} & \textit{\tentry{0.58}{0.06}\textsuperscript{\textbf{*}}} & \tentry{0.61}{0.08}\textsuperscript{\textbf{*}} & \tentry{0.52}{0.09} & \tentry{0.62}{0.04}\textsuperscript{\textbf{*}} & \tentry{0.62}{0.05}\textsuperscript{\textbf{*}} & \tentry{0.47}{0.09} & \tentry{0.57}{0.11} & \tentry{0.50}{0.08} \\
        & \multicolumn{1}{l}{CBM-joint} & \tentry{0.55}{0.06} & \tentry{0.46}{0.06} & \tentry{0.66}{0.06}\textsuperscript{\textbf{*}} & \tentry{0.47}{0.06} & \textit{\tentry{0.64}{0.04}\textsuperscript{\textbf{*}}} & \tentry{0.53}{0.07} & \tentry{0.50}{0.07} & \tentry{0.58}{0.10}\textsuperscript{\textbf{*}} & \tentry{0.49}{0.04} \\
        \cmidrule{2-11} & \multicolumn{1}{l}{MVCBM-seq-avg} & \tentry{0.54}{0.08} & \tentry{0.55}{0.04} & \textbf{\tentry{0.72}{0.07}\textsuperscript{\textbf{*}}} & \tentry{0.62}{0.04}\textsuperscript{\textbf{*}} & \tentry{0.50}{0.05} & \tentry{0.64}{0.06}\textsuperscript{\textbf{*}} & \tentry{0.51}{0.10} & \tentry{0.47}{0.11} & \tentry{0.54}{0.10} \\
        & \multicolumn{1}{l}{MVCBM-seq-LSTM}   & \textbf{\tentry{0.82}{0.04}\textsuperscript{\textbf{*}}} & \tentry{0.53}{0.04} & \tentry{0.62}{0.04}\textsuperscript{\textbf{*}} & \textbf{\tentry{0.69}{0.04}\textsuperscript{\textbf{*}}} & \tentry{0.62}{0.05}\textsuperscript{\textbf{*}} & \textbf{\tentry{0.72}{0.05}\textsuperscript{\textbf{*}}} & \textbf{\tentry{0.64}{0.06}\textsuperscript{\textbf{*}}} & \textbf{\tentry{0.78}{0.03}\textsuperscript{\textbf{*}}} & \textbf{\tentry{0.70}{0.06}\textsuperscript{\textbf{*}}} \\
        & \multicolumn{1}{l}{MVCBM-joint-avg}   & \tentry{0.54}{0.09} & \tentry{0.51}{0.06} & \tentry{0.70}{0.06}\textsuperscript{\textbf{*}} & \tentry{0.59}{0.08}\textsuperscript{\textbf{*}} & \tentry{0.61}{0.06}\textsuperscript{\textbf{*}} & \tentry{0.62}{0.05}\textsuperscript{\textbf{*}} & \tentry{0.54}{0.15} & \tentry{0.48}{0.14} & \tentry{0.55}{0.12} \\
        & \multicolumn{1}{l}{MVCBM-joint-LSTM} & \textbf{\tentry{0.82}{0.03}\textsuperscript{\textbf{*}}} & \tentry{0.48}{0.06} & \tentry{0.66}{0.07}\textsuperscript{\textbf{*}} & \tentry{0.64}{0.06}\textsuperscript{\textbf{*}} & \textbf{\tentry{0.65}{0.05}\textsuperscript{\textbf{*}}} & \tentry{0.64}{0.09}\textsuperscript{\textbf{*}} & \tentry{0.47}{0.09} & \tentry{0.61}{0.14} & \textit{\tentry{0.65}{0.05}\textsuperscript{\textbf{*}}} \\
        \cmidrule{2-11} & \multicolumn{1}{l}{SSMVCBM-avg} & \tentry{0.53}{0.06}\textsuperscript{\textbf{*}} & \tentry{0.56}{0.08}\textsuperscript{\textbf{*}} & \textit{\tentry{0.71}{0.05}\textsuperscript{\textbf{*}}} & \tentry{0.60}{0.06}\textsuperscript{\textbf{*}} & \tentry{0.51}{0.05} & \tentry{0.64}{0.09}\textsuperscript{\textbf{*}} & \tentry{0.46}{0.08} & \tentry{0.48}{0.09} & \tentry{0.53}{0.03} \\
        & \multicolumn{1}{l}{SSMVCBM-LSTM} & \textit{\tentry{0.77}{0.10}\textsuperscript{\textbf{*}}} & \textbf{\tentry{0.59}{0.08}} & \tentry{0.70}{0.06}\textsuperscript{\textbf{*}} & \textit{\tentry{0.67}{0.07}\textsuperscript{\textbf{*}}} & \textbf{\tentry{0.65}{0.07}\textsuperscript{\textbf{*}}} & \textit{\tentry{0.67}{0.05}\textsuperscript{\textbf{*}}} & \textit{\tentry{0.62}{0.08}\textsuperscript{\textbf{*}}} & \textit{\tentry{0.74}{0.15}\textsuperscript{\textbf{*}}} & \tentry{0.64}{0.11}\textsuperscript{\textbf{*}} \\
        \midrule
        \multirow{11}{20mm}{\textbf{AUPR}}
        & \multicolumn{1}{l}{Random} & 0.72 & 0.49 & 0.19 & 0.23 & 0.51 & 0.26 & 0.16 & 0.13 & 0.14 \\
        \cmidrule{2-11} & \multicolumn{1}{l}{CBM-seq} & \tentry{0.75}{0.03} & \textit{\tentry{0.58}{0.05}\textsuperscript{\textbf{*}}} & \tentry{0.34}{0.09}\textsuperscript{\textbf{*}} & \tentry{0.24}{0.05} & \tentry{0.64}{0.04}\textsuperscript{\textbf{*}} & \tentry{0.35}{0.06}\textsuperscript{\textbf{*}} & \tentry{0.18}{0.05} & \tentry{0.19}{0.07} & \tentry{0.15}{0.03} \\
        & \multicolumn{1}{l}{CBM-joint} & \tentry{0.77}{0.05} & \tentry{0.47}{0.04} & \textit{\tentry{0.37}{0.09}\textsuperscript{\textbf{*}}} & \tentry{0.25}{0.06} & \tentry{0.64}{0.05}\textsuperscript{\textbf{*}} & \tentry{0.30}{0.07} & \tentry{0.17}{0.04} & \tentry{0.18}{0.06} & \tentry{0.18}{0.08} \\
        \cmidrule{2-11} & \multicolumn{1}{l}{MVCBM-seq-avg} & \tentry{0.75}{0.05} & \textit{\tentry{0.58}{0.06}\textsuperscript{\textbf{*}}} & \textbf{\tentry{0.42}{0.07}\textsuperscript{\textbf{*}}} & \tentry{0.33}{0.06}\textsuperscript{\textbf{*}} & \tentry{0.53}{0.05} & \tentry{0.41}{0.08}\textsuperscript{\textbf{*}} & \tentry{0.21}{0.05} & \tentry{0.13}{0.05} & \textit{\tentry{0.24}{0.12}} \\
        & \multicolumn{1}{l}{MVCBM-seq-LSTM}   & \textit{\tentry{0.91}{0.04}\textsuperscript{\textbf{*}}} & \tentry{0.55}{0.04}\textsuperscript{\textbf{*}} & \tentry{0.33}{0.08}\textsuperscript{\textbf{*}} & \textbf{\tentry{0.40}{0.06}\textsuperscript{\textbf{*}}} & \textit{\tentry{0.65}{0.03}\textsuperscript{\textbf{*}}} & \textbf{\tentry{0.50}{0.11}\textsuperscript{\textbf{*}}} & \textit{\tentry{0.23}{0.05}\textsuperscript{\textbf{*}}} & \textit{\tentry{0.27}{0.05}\textsuperscript{\textbf{*}}} & \textbf{\tentry{0.26}{0.07}\textsuperscript{\textbf{*}}} \\
        & \multicolumn{1}{l}{MVCBM-joint-avg} & \tentry{0.74}{0.06} & \tentry{0.51}{0.07} & \textbf{\tentry{0.42}{0.09}\textsuperscript{\textbf{*}}} & \tentry{0.28}{0.07} & \tentry{0.59}{0.06}\textsuperscript{\textbf{*}} & \tentry{0.35}{0.05}\textsuperscript{\textbf{*}} & \tentry{0.22}{0.06} & \tentry{0.22}{0.13} & \tentry{0.21}{0.08} \\
        & \multicolumn{1}{l}{MVCBM-joint-LSTM} & \textbf{\tentry{0.92}{0.02}\textsuperscript{\textbf{*}}} & \tentry{0.49}{0.05} & \textit{\tentry{0.37}{0.11}\textsuperscript{\textbf{*}}} & \tentry{0.32}{0.07}\textsuperscript{\textbf{*}} & \textit{\tentry{0.65}{0.06}\textsuperscript{\textbf{*}}} & \tentry{0.39}{0.07}\textsuperscript{\textbf{*}} & \tentry{0.20}{0.06} & \tentry{0.17}{0.07} & \tentry{0.21}{0.06}\textsuperscript{\textbf{*}} \\
        \cmidrule{2-11} & \multicolumn{1}{l}{SSMVCBM-avg} & \tentry{0.73}{0.05} & \textit{\tentry{0.58}{0.07}\textsuperscript{\textbf{*}}} & \tentry{0.36}{0.05}\textsuperscript{\textbf{*}} & \tentry{0.28}{0.04}\textsuperscript{\textbf{*}} & \tentry{0.53}{0.05} & \tentry{0.37}{0.09}\textsuperscript{\textbf{*}} & \tentry{0.20}{0.06} & \tentry{0.13}{0.02} & \textit{\tentry{0.24}{0.06}\textsuperscript{\textbf{*}}} \\
        & \multicolumn{1}{l}{SSMVCBM-LSTM} & \tentry{0.88}{0.06}\textsuperscript{\textbf{*}} & \textbf{\tentry{0.60}{0.06}\textsuperscript{\textbf{*}}} & \textbf{\tentry{0.42}{0.06}\textsuperscript{\textbf{*}}} & \textit{\tentry{0.39}{0.09}\textsuperscript{\textbf{*}}} & \textbf{\tentry{0.67}{0.07}\textsuperscript{\textbf{*}}} & \textit{\tentry{0.43}{0.10}\textsuperscript{\textbf{*}}} & \textbf{\tentry{0.24}{0.08}} & \textbf{\tentry{0.30}{0.13}\textsuperscript{\textbf{*}}} & \tentry{0.20}{0.05}\textsuperscript{\textbf{*}} \\
        \bottomrule
    \end{tabular}
    \end{center}
\end{table*}
\end{landscape}

==> src/tables/contingency.tex <==
\begin{table}[h]
    \centering
    \caption{The contingency table of the pediatric appendicitis dataset of the management (M) by severity (S) stratified by the diagnosis (D).}
    \label{tab:contingency}
    \footnotesize 
    \begin{tabular}{lccc}
        \toprule%
        & \multicolumn{3}{@{}c@{}}{\textbf{D: \textit{appendicitis}}} \\ \cmidrule{2-4}
        \diagbox{{\textbf{M}}}{{\textbf{S}}} & \textit{complicated} & \makecell{\textit{uncomplicated}} & \textbf{Total} \\
        \toprule
        \textit{surgical} & 97 & 135 & 232 \\
        \textit{conservative} & 0 & 151 & 151 \\
        \cline{1-4}
        \textbf{Total} & 97 & 286 & 383 \\
        \bottomrule
        & \\
        & \\
        \toprule
        & \multicolumn{3}{@{}c@{}}{\textbf{D: \textit{no appendicitis}}} \\\cmidrule{2-4}
        \diagbox{{\textbf{M}}}{{\textbf{S}}} & \textit{complicated} & \makecell{\textit{uncomplicated}} & \textbf{Total} \\
        \toprule
        \textit{surgical} & 0 & 2 & 2 \\
        \textit{conservative} & 0 & 194 & 194 \\
        \cline{1-4}
        \textbf{Total} & 0 & 196 & 196 \\
        \bottomrule
    \end{tabular}
\end{table}

==> src/tables/hyperparameters_1.tex <==
\begin{landscape}
\begin{table}[h!]
    \footnotesize
    \centering
    \caption{Final hyperparameter values used to train models on the \textbf{synthetic nonlinear data}.}
    \label{tab:parameters_synthetic} 
    \centering
    \begin{tabular}{l c c c c c c c c c c c c} 
        \toprule
        \multirow{2}{*}{\raisebox{-\heavyrulewidth}{\textbf{Model}}} & \multicolumn{11}{c}{\textbf{Hyperparameter}}\\
        \cmidrule{2-13} & $E_{\boldsymbol{c}}$ & $C$ & $E_{\boldsymbol{z}}$ & $E_a$ & $E_y$ & $\eta_{\boldsymbol{c}}$ & $\eta_{\boldsymbol{z}}$ & $\eta_a$ & $\eta_y$ & $B$ & $\alpha$ & $\lambda$ \\
        \midrule
        MLP & --- & --- & --- & --- & 150 & --- & --- & --- & 1.0e-3 & 64 & --- & --- \\
        \midrule
        CBM-seq & 100 & --- & --- & --- & 50 & 1.0e-3 & --- & --- & 1.0e-3 & 64 & --- & --- \\
        CBM-joint & --- & --- & --- & --- & 120 & --- & ---- & --- & 1.0e-4 & 64 & 1.0 & --- \\
        \midrule
        MVBM-avg & --- & --- & --- & --- & 150 & --- & --- & --- & 1.0e-3 & 64 & --- & --- \\
        MVBM-LSTM & --- & --- & --- & --- & 150 & --- & ---- & --- & 1.0e-3 & 64 & --- & --- \\
        \midrule
        MVCBM-seq-avg & 100 & --- & --- & --- & 50 & 1.0e-3 & --- & --- & 1.0e-3 & 64 & --- & ---\\
        MVCBM-seq-LSTM & 100 & --- & --- & --- & 50 & 1.0e-3 & --- & --- & 1.0e-3 & 64 & --- & --- \\
        MVCBM-joint-avg & --- & --- & --- & --- & 120 & --- & --- & --- & 1.0e-4 & 64 & 1.0 & --- \\
        MVCBM-joint-LSTM & --- & --- & --- & --- & 120 & --- & --- & --- & 1.0e-4 & 64 & 1.0 & --- \\
        \midrule
        SSMVCBM-avg & 100 & 7 & 30 & 30 & 50 & 1.0e-3 & 1.0e-3 & 1.0e-3  & 1.0e-3 & 64 & --- & 1.0e-2 \\
        SSMVCBM-LSTM & 100 & 7 & 30 & 30 & 50 & 1.0e-3 & 1.0e-3 & 1.0e-3  & 1.0e-3 & 64 & --- & 1.0e-2 \\
        \bottomrule
    \end{tabular}

    \vspace{0.25cm}
    
    {
    \begin{flushleft}
    \footnotesize
    \textbf{Note:} $E_{\boldsymbol{c}}$: the number of training epochs for the concept model; $C$: the number of iterations in the adversarial training procedure for the SSMVCBM; $E_{\boldsymbol{z}}$: the number of training epochs for the representation learning module; $E_{a}$: the number of training epochs for the adversary; $E_y$: the number of training epochs for the target model or the full model; $\eta_{\boldsymbol{c}}$: the learning rate (LR) for the concept model; $\eta_{\boldsymbol{z}}$: the LR for the representation learning module; $\eta_a$: the LR for the adversary; $\eta_y$: the LR for the target or the full model; $B$: the mini-batch size; $\alpha$: a parameter controlling the trade-off between target and concept prediction in the joint optimization; $\lambda$: the weight of the adversarial regularizer in the loss function of the SSMVCBM.
    \end{flushleft}
    }
\end{table}
\end{landscape}

\begin{landscape}
\begin{table}[h!]
    \footnotesize
    \centering
    \caption{Final hyperparameter values used to train models on the \textbf{multiview animals with attributes}.}
    \label{tab:parameters_mvawa}
    \begin{tabular}{l c c c c c c c c c c c c} 
        \toprule
        \multirow{2}{*}{\raisebox{-\heavyrulewidth}{\textbf{Model}}} & \multicolumn{11}{c}{\textbf{Hyperparameter}}\\
        \cmidrule{2-13} & $E_{\boldsymbol{c}}$ & $C$ & $E_{\boldsymbol{z}}$ & $E_a$ & $E_y$ & $\eta_{\boldsymbol{c}}$ & $\eta_{\boldsymbol{z}}$ & $\eta_a$ & $\eta_y$ & $B$ & $\alpha$ & $\lambda$ \\
        \midrule
        ResNet-18 & --- & --- & --- & --- & 120 & --- & --- & --- & 1.0e-4 & 64 & --- & --- \\
        \midrule
        CBM-seq & 25 & --- & --- & --- & 20 & 1.0e-4 & --- & --- & 1.0e-2 & 64 & --- \\
        CBM-joint & --- & --- & --- & --- & 120 & --- & --- & --- & 1.0e-4 & 64 & 1.0 & --- \\
        \midrule
        MVBM-avg & --- & --- & --- & --- & 120 & --- & --- & --- & 1.0e-4 & 64 & --- & --- \\
        MVBM-LSTM & --- & --- & --- & --- & 120 & --- & --- & --- & 1.0e-4 & 64 & --- & --- \\
        \midrule
        MVCBM-seq-avg & 25 & --- & --- & --- & 20 & 1.0e-4 & --- & --- & 1.0e-2 & 64 & --- & --- \\
        MVCBM-seq-LSTM & 25 & --- & --- & --- & 20 & 1.0e-4 & --- & --- & 1.0e-2 & 64 & --- & --- \\
        MVCBM-joint-avg & --- & --- & --- & --- & 120 & --- & --- & --- & 1.0e-4 & 64 & 1.0 & --- \\
        MVCBM-joint-LSTM & --- & --- & --- & --- & 120 & --- & --- & --- & 1.0e-4 & 64 & 1.0 & --- \\
        \midrule
        SSMVCBM-avg & 25 & 7 & 15 & 10 & 20 & 1.0e-4 & 1.0e-4 & 1.0e-2 & 1.0e-2 & 64 & --- & 1.0e-2 \\
        SSMVCBM-LSTM & 25 & 7 & 15 & 10 & 20 & 1.0e-4 & 1.0e-4 & 1.0e-2 & 1.0e-2 & 64 & --- & 1.0e-2 \\
        \bottomrule
    \end{tabular}

    \vspace{0.25cm}
    
    {
    \begin{flushleft}
    \footnotesize
    \textbf{Note:} $E_{\boldsymbol{c}}$: the number of training epochs for the concept model; $C$: the number of iterations in the adversarial training procedure for the SSMVCBM; $E_{\boldsymbol{z}}$: the number of training epochs for the representation learning module; $E_{a}$: the number of training epochs for the adversary; $E_y$: the number of training epochs for the target model or the full model; $\eta_{\boldsymbol{c}}$: the learning rate (LR) for the concept model; $\eta_{\boldsymbol{z}}$: the LR for the representation learning module; $\eta_a$: the LR for the adversary; $\eta_y$: the LR for the target or the full model; $B$: the mini-batch size; $\alpha$: a parameter controlling the trade-off between target and concept prediction in the joint optimization; $\lambda$: the weight of the adversarial regularizer in the loss function of the SSMVCBM.
    \end{flushleft}
    }
\end{table}
\end{landscape}

==> src/tables/hyperparameters_2.tex <==
\begin{landscape}
\begin{table}[h!]
    \footnotesize
    \centering
    \caption{Final hyperparameter values used to train models on the \textbf{appendicitis} data with the \textbf{diagnosis} as the target.}
    \label{tab:parameters_app_diagnosis}
    \begin{tabular}{l c c c c c c c c c c c c} 
        \toprule
        \multirow{2}{*}{\raisebox{-\heavyrulewidth}{\textbf{Model}}} & \multicolumn{11}{c}{\textbf{Hyperparameter}}\\
        \cmidrule{2-13} & $E_{\boldsymbol{c}}$ & $C$ & $E_{\boldsymbol{z}}$ & $E_a$ & $E_y$ & $\eta_{\boldsymbol{c}}$ & $\eta_{\boldsymbol{z}}$ & $\eta_a$ & $\eta_y$ & $B$ & $\alpha$ & $\lambda$ \\
        \midrule
        ResNet-18 & --- & --- & --- & --- & 120 & --- & --- & --- & 1.0e-4 & 4 & --- & --- \\
        \midrule
        CBM-seq & 25 & --- & --- & --- & 20 & 1.0e-4 & --- & --- & 1.0e-2 & 4 & --- & --- \\
        CBM-joint & --- & --- & --- & --- & 120 & --- & --- & --- & 1.0e-4 & 4 & 1.0 & --- \\
        \midrule
        MVBM-avg & --- & --- & --- & --- & 120 & --- & --- & --- & 1.0e-4 & 4 & --- & --- \\
        MVBM-LSTM & --- & --- & --- & --- & 50 & --- & --- & --- & 1.0e-4 & 4 & --- & --- \\
        \midrule
        MVCBM-seq-avg & 20 & --- & --- & --- & 20 & 1.0e-4 & --- & --- & 1.0e-2 & 4 & --- & --- \\
        MVCBM-seq-LSTM & 20 & --- & --- & --- & 20 & 1.0e-4 & --- & --- & 1.0e-2 & 4 & --- & --- \\
        MVCBM-joint-avg & --- & --- & --- & --- & 120 & --- & --- & --- & 1.0e-4 & 4 & 1.0 & --- \\
        MVCBM-joint-LSTM & --- & --- & --- & --- & 40 & --- & --- & --- & 1.0e-3 & 4 & 1.0 & --- \\
        \midrule
        SSMVCBM-avg & 20 & 7 & 15 & 10 & 20 & 1.0e-4 & 1.0e-4 & 1.0e-2 & 1.0e-2 & 8 & --- & 1.0e-2 \\
        SSMVCBM-LSTM & 20 & 7 & 15 & 10 & 20 & 1.0e-4 & 1.0e-4 & 1.0e-2 & 1.0e-2 & 8 & --- & 1.0e-2 \\
        \bottomrule
    \end{tabular}

    \vspace{0.25cm}
    
    {
    \begin{flushleft}
    \footnotesize
    \textbf{Note:} $E_{\boldsymbol{c}}$: the number of training epochs for the concept model; $C$: the number of iterations in the adversarial training procedure for the SSMVCBM; $E_{\boldsymbol{z}}$: the number of training epochs for the representation learning module; $E_{a}$: the number of training epochs for the adversary; $E_y$: the number of training epochs for the target model or the full model; $\eta_{\boldsymbol{c}}$: the learning rate (LR) for the concept model; $\eta_{\boldsymbol{z}}$: the LR for the representation learning module; $\eta_a$: the LR for the adversary; $\eta_y$: the LR for the target or the full model; $B$: the mini-batch size; $\alpha$: a parameter controlling the trade-off between target and concept prediction in the joint optimization; $\lambda$: the weight of the adversarial regularizer in the loss function of the SSMVCBM.
    \end{flushleft}
    }
\end{table}
\end{landscape}

\begin{landscape}
\begin{table}[h!]
    \footnotesize
    \centering
    \caption{Final hyperparameter values used to train models on the \textbf{appendicitis} data with the \textbf{management} as the target.}
    \label{tab:parameters_app_management}
    \begin{tabular}{l c c c c c c c c c c c c} 
        \toprule
        \multirow{2}{*}{\raisebox{-\heavyrulewidth}{\textbf{Model}}} & \multicolumn{11}{c}{\textbf{Hyperparameter}}\\
        \cmidrule{2-13} & $E_{\boldsymbol{c}}$ & $C$ & $E_{\boldsymbol{z}}$ & $E_a$ & $E_y$ & $\eta_{\boldsymbol{c}}$ & $\eta_{\boldsymbol{z}}$ & $\eta_a$ & $\eta_y$ & $B$ & $\alpha$ & $\lambda$ \\
        \midrule
        ResNet-18 & --- & --- & --- & --- & 120 & --- & --- & --- & 1.0e-4 & 4 & --- & --- \\
        \midrule
        CBM-seq & 25 & --- & --- & --- & 20 & 1.0e-4 & --- & --- & 1.0e-2 & 4 & --- & --- \\
        CBM-joint & --- & --- & --- & --- & 120 & --- & --- & --- & 1.0e-4 & 4 & 1.0 & --- \\
        \midrule
        MVBM-avg & --- & --- & --- & --- & 120 & --- & --- & --- & 1.0e-4 & 4 & --- & --- \\
        MVBM-LSTM & --- & --- & --- & --- & 50 & --- & --- & --- & 1.0e-4 & 4 & --- & --- \\
        \midrule
        MVCBM-seq-avg & 20 & --- & --- & --- & 20 & 1.0e-4 & --- & --- & 1.0e-2 & 4 & --- & --- \\
        MVCBM-seq-LSTM & 20 & --- & --- & --- & 20 & 1.0e-4 & --- & --- & 1.0e-2 & 4 & --- & --- \\
        MVCBM-joint-avg & --- & --- & --- & --- & 120 & --- & --- & --- & 1.0e-4 & 4 & 1.0 & --- \\
        MVCBM-joint-LSTM & --- & --- & --- & --- & 120 & --- & --- & --- & 1.0e-4 & 4 & 1.0 & --- \\
        \midrule
        SSMVCBM-avg & 20 & 7 & 15 & 10 & 20 & 1.0e-4 & 1.0e-4 & 1.0e-2 & 1.0e-2 & 8 & --- & 1.0e-2 \\
        SSMVCBM-LSTM & 20 & 7 & 15 & 10 & 20 & 1.0e-4 & 1.0e-4 & 1.0e-2 & 1.0e-2 & 8 & --- & 1.0e-2 \\
        \bottomrule
    \end{tabular}

    \vspace{0.25cm}
    
    {
    \begin{flushleft}
    \footnotesize
    \textbf{Note:} $E_{\boldsymbol{c}}$: the number of training epochs for the concept model; $C$: the number of iterations in the adversarial training procedure for the SSMVCBM; $E_{\boldsymbol{z}}$: the number of training epochs for the representation learning module; $E_{a}$: the number of training epochs for the adversary; $E_y$: the number of training epochs for the target model or the full model; $\eta_{\boldsymbol{c}}$: the learning rate (LR) for the concept model; $\eta_{\boldsymbol{z}}$: the LR for the representation learning module; $\eta_a$: the LR for the adversary; $\eta_y$: the LR for the target or the full model; $B$: the mini-batch size; $\alpha$: a parameter controlling the trade-off between target and concept prediction in the joint optimization; $\lambda$: the weight of the adversarial regularizer in the loss function of the SSMVCBM.
    \end{flushleft}
    }
\end{table}
\end{landscape}

\begin{landscape}
\begin{table}[h!]
    \footnotesize
    \centering
    \caption{Final hyperparameter values used to train models on the \textbf{appendicitis} data with the \textbf{severity} as the target.}
    \label{tab:parameters_app_severity}
    \begin{tabular}{l c c c c c c c c c c c c} 
        \toprule
        \multirow{2}{*}{\raisebox{-\heavyrulewidth}{\textbf{Model}}} & \multicolumn{11}{c}{\textbf{Hyperparameter}}\\
        \cmidrule{2-13} & $E_{\boldsymbol{c}}$ & $C$ & $E_{\boldsymbol{z}}$ & $E_a$ & $E_y$ & $\eta_{\boldsymbol{c}}$ & $\eta_{\boldsymbol{z}}$ & $\eta_a$ & $\eta_y$ & $B$ & $\alpha$ & $\lambda$ \\
        \midrule
        ResNet-18 & --- & --- & --- & --- & 120 & --- & --- & --- & 1.0e-4 & 4 & --- & --- \\
        \midrule
        CBM-seq & 25 & --- & --- & --- & 20 & 1.0e-4 & --- & --- & 1.0e-2 & 4 & --- & --- \\
        CBM-joint & --- & --- & --- & --- & 120 & --- & --- & --- & 1.0e-4 & 4 & 1.0 & --- \\
        \midrule
        MVBM-avg & --- & --- & --- & --- & 120 & --- & --- & --- & 1.0e-4 & 4 & --- & --- \\
        MVBM-LSTM & --- & --- & --- & --- & 70 & --- & --- & --- & 1.0e-4 & 4 & --- & --- \\
        \midrule
        MVCBM-seq-avg & 30 & --- & --- & --- & 40 & 1.0e-4 & --- & --- & 1.0e-3 & 4 & --- & --- \\
        MVCBM-seq-LSTM & 30 & --- & --- & --- & 40 & 1.0e-4 & --- & --- & 1.0e-3 & 4 & --- & --- \\
        MVCBM-joint-avg & --- & --- & --- & --- & 100 & --- & --- & --- & 1.0e-4 & 4 & 1.0 & --- \\
        MVCBM-joint-LSTM & --- & --- & --- & --- & 100 & --- & --- & --- & 1.0e-4 & 4 & 1.0 & --- \\
        \midrule
        SSMVCBM-avg & 20 & 7 & 15 & 10 & 20 & 1.0e-4 & 1.0e-4 & 1.0e-2 & 1.0e-2 & 8 & --- & 1.0e-2 \\
        SSMVCBM-LSTM & 20 & 7 & 15 & 10 & 20 & 1.0e-4 & 1.0e-4 & 1.0e-2 & 1.0e-2 & 8 & --- & 1.0e-2 \\
        \bottomrule
    \end{tabular}

    \vspace{0.25cm}
    
    {
    \begin{flushleft}
    \footnotesize
    \textbf{Note:} $E_{\boldsymbol{c}}$: the number of training epochs for the concept model; $C$: the number of iterations in the adversarial training procedure for the SSMVCBM; $E_{\boldsymbol{z}}$: the number of training epochs for the representation learning module; $E_{a}$: the number of training epochs for the adversary; $E_y$: the number of training epochs for the target model or the full model; $\eta_{\boldsymbol{c}}$: the learning rate (LR) for the concept model; $\eta_{\boldsymbol{z}}$: the LR for the representation learning module; $\eta_a$: the LR for the adversary; $\eta_y$: the LR for the target or the full model; $B$: the mini-batch size; $\alpha$: a parameter controlling the trade-off between target and concept prediction in the joint optimization; $\lambda$: the weight of the adversarial regularizer in the loss function of the SSMVCBM.
    \end{flushleft}
    }
\end{table}
\end{landscape}

==> src/tables/predictive_perf_app.tex <==
\begin{table*}[h!]
    \footnotesize
    \centering
    \caption{Models' test-set performance at predicting diagnosis, management and severity. Test-set AUROCs and AUPRs are reported as averages and standard deviations across ten independent initialization. Bold indicates the best result; italics indicates the second best.}
    \label{tab:appendicitis_target_res} 
    \begin{tabular}{lm{1.2cm}m{1.2cm}cm{1.2cm}m{1.2cm}cm{1.2cm}m{1.2cm}}
        \toprule
        \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Diagnosis}} &  & \multicolumn{2}{c}{\textbf{Management}} &  & \multicolumn{2}{c}{\textbf{Severity}}\\
        \cmidrule{2-3}\cmidrule{5-6}\cmidrule{8-9} & \multicolumn{1}{c}{\textbf{AUROC}} & \multicolumn{1}{c}{\textbf{AUPR}} &  & \multicolumn{1}{c}{\textbf{AUROC}} & \multicolumn{1}{c}{\textbf{AUPR}} &  & \multicolumn{1}{c}{\textbf{AUROC}} & \multicolumn{1}{c}{\textbf{AUPR}} \\
        \toprule
        Random & 0.50 & 0.75 &  & 0.50 & 0.47 &  & 0.50 & 0.23 \\
        \midrule
        Radiomics + RF & \tentry{0.63}{0.01} & \tentry{0.82}{0.01} &  & \tentry{0.59}{0.01} & \tentry{0.51}{0.02} &  & \textbf{\tentry{0.78}{0.01}} & \tentry{0.54}{0.02} \\
        \midrule
        ResNet-18 & \tentry{0.70}{0.07} & \tentry{0.88}{0.04} &  & \tentry{0.69}{0.07} & \textit{\tentry{0.71}{0.08}} &  & \tentry{0.73}{0.10} & \tentry{0.52}{0.10} \\
        \midrule
        CBM-seq & \tentry{0.64}{0.06} & \tentry{0.84}{0.04} &  & \tentry{0.68}{0.05} & \tentry{0.68}{0.05} &  & \tentry{0.66}{0.06} & \tentry{0.41}{0.08} \\
        CBM-joint & \tentry{0.62}{0.04} & \tentry{0.83}{0.04} &  & \tentry{0.66}{0.06} & \tentry{0.68}{0.04} &  & \tentry{0.68}{0.06} & \tentry{0.44}{0.08} \\
        \midrule
        MVBM-avg & \textit{\tentry{0.76}{0.05}} & \tentry{0.89}{0.04} &  & \textit{\tentry{0.71}{0.04}} & \tentry{0.69}{0.04} &  & \tentry{0.71}{0.12} & \textbf{\tentry{0.59}{0.11}} \\
        MVBM-LSTM & \textit{\tentry{0.76}{0.04}} & \textit{\tentry{0.91}{0.02}} &  & \tentry{0.67}{0.04} & \tentry{0.61}{0.04} &  & \tentry{0.74}{0.13} & \textit{\tentry{0.58}{0.12}} \\
        \midrule
        MVCBM-seq-avg & \tentry{0.67}{0.05} & \tentry{0.85}{0.05} &  & \tentry{0.58}{0.05} & \tentry{0.62}{0.06} &  & \textit{\tentry{0.75}{0.07}} & \tentry{0.56}{0.12} \\
        MVCBM-seq-LSTM & \tentry{0.73}{0.03} & \tentry{0.89}{0.01} &  & \tentry{0.57}{0.03} & \tentry{0.53}{0.04} &  & \tentry{0.70}{0.11} & \tentry{0.48}{0.16} \\
        MVCBM-joint-avg & \tentry{0.66}{0.09} & \tentry{0.84}{0.06} &  & \tentry{0.69}{0.06} & \tentry{0.66}{0.11} &  & \tentry{0.70}{0.06} & \tentry{0.53}{0.11} \\
        MVCBM-joint-LSTM & \tentry{0.72}{0.02} & \tentry{0.88}{0.02} &  & \tentry{0.57}{0.05} & \tentry{0.50}{0.04} &  & \tentry{0.65}{0.07} & \tentry{0.37}{0.10} \\
        \midrule
        SSMVCBM-avg & \textbf{\tentry{0.80}{0.03}} & \textbf{\tentry{0.92}{0.02}} &  & \textbf{\tentry{0.72}{0.05}} & \textbf{\tentry{0.72}{0.04}} &  & \tentry{0.73}{0.07} & \tentry{0.57}{0.09} \\
        SSMVCBM-LSTM & \textbf{\tentry{0.80}{0.06}} & \textbf{\tentry{0.92}{0.04}} &  & \tentry{0.70}{0.03} & \tentry{0.67}{0.06} &  & \textbf{\tentry{0.78}{0.05}} & \textit{\tentry{0.58}{0.10}} \\
        \bottomrule
    \end{tabular}
\end{table*}

==> src/tables/predictive_perf_mvawa.tex <==
\begin{table}[ht!]
\centering
\caption{Target and concept prediction results for MVCBM and SSMVCBM models and several baselines under different optimization procedures and fusion functions on the MVAwA data with the full concept set. The performance is reported as averages and standard deviations of the AUROC across ten independent simulations. Herein, ``seq'' and ``joint'' denote sequential and joint optimization, respectively; whereas ``avg'' and ``LSTM'' stand for the averaging- and LSTM-based fusion.}
\label{tab:mvawa_full_res}
\begin{tabular}{lm{1.25cm}cm{1.25cm}}
    \toprule
    \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{AUROC}}\\
    \cmidrule{2-4} &
    \multicolumn{1}{c}{\textbf{Target}} & & \multicolumn{1}{c}{\textbf{Concepts}} \\
    \toprule
    Random & 0.50 &  & 0.50 \\
    \midrule
    ResNet-18 & \tentry{0.85}{0.01} & & --- \\
    \midrule
    CBM-seq & \tentry{0.81}{0.01} & & \tentry{0.86}{0.01} \\
    CBM-joint & \tentry{0.84}{0.01} & & \tentry{0.85}{0.01} \\
    \midrule
    MVBM-avg & \tentry{0.96}{0.00} & & --- \\
    MVBM-LSTM & \tentry{0.95}{0.00} & & --- \\
    \midrule
    MVCBM-seq-avg & \tentry{0.95}{0.01} & & \tentry{0.97}{0.00} \\
    MVCBM-seq-LSTM & \tentry{0.92}{0.01} & & \tentry{0.95}{0.00} \\
    MVCBM-joint-avg & \tentry{0.94}{0.01} & & \tentry{0.96}{0.00} \\
    MVCBM-joint-LSTM & \tentry{0.95}{0.00} & & \tentry{0.96}{0.01} \\
    \midrule
    SSMVCBM-avg & \tentry{0.94}{0.00} & & \tentry{0.97}{0.00} \\
    SSMVCBM-LSTM & \tentry{0.92}{0.01} & & \tentry{0.95}{0.00} \\
    \bottomrule
\end{tabular}
\end{table}
